GenTKG: Generative Forecasting on Temporal Knowledge Graph with Large Language Models

The rapid advancements in large language models (LLMs) have ignited interest in the temporal knowledge graph (tKG) domain, where conventional embedding-based and rule-based methods dominate. The question remains open of whether pre-trained LLMs can understand structured temporal relational data and replace them as the foundation model for temporal relational forecasting. Therefore, we bring temporal knowledge forecasting into the generative setting. However, challenges occur in the huge chasms between complex temporal graph data structure and sequential natural expressions LLMs can handle, and between the enormous data sizes of tKGs and heavy computation costs of finetuning LLMs. To address these challenges, we propose a novel retrieval-augmented generation framework named GenTKG combining a temporal logical rule-based retrieval strategy and few-shot parameter-efficient instruction tuning to solve the above challenges, respectively. Extensive experiments have shown that GenTKG outperforms conventional methods of temporal relational forecasting with low computation resources using extremely limited training data as few as 16 samples. GenTKG also highlights remarkable cross-domain generalizability with outperforming performance on unseen datasets without re-training, and in-domain generalizability regardless of time split in the same dataset. Our work reveals the huge potential of LLMs in the tKG domain and opens a new frontier for generative forecasting on tKGs. Code and data are released here: https://github.com/mayhugotong/GenTKG.

==> latex/2_related.tex <==
\section{Related Works}

%The answers are provided as either entity identifiers, natural languages or both. To answer such questions, models usually retrieve a subgraph from large scale knowledge graphs, then perform a classification on them to get the correct entities.
\label{sec:appendix}
\textbf{Temporal Knowledge Graphs}
Temporal knowledge graphs (tKGs) are multi-relational, directed graphs with labeled timestamped edges between entities (nodes). Let $\mathcal{E}$ and $\mathcal{P}$ represent a finite set of entities and predicates. A quadruple $(e_s, r, e_o, t)$ represents a timestamped and labeled edge between a subject entity $e_s \in \mathcal{E}$ and an object entity $e_o \in \mathcal{E}$ at a timestamp $t \in \mathcal{T}$. Let $\mathcal{F}$ represent the set of all true quadruples, i.e., real
events in the world, the temporal knowledge graph forecasting is the task of predicting missing object entity at timestamp $t$, i.e. $(e_s, r, ?, t)$ based on a set of observed facts $\mathcal{O}$ before $t$, which is a subset of $\mathcal{F}$.  Current methods can be categorized into two streams. On the one hand, embedding-based models learn representations of the quadruples with carefully designed embedding models\cite{han2020explainable, goel2020diachronic, sun2021timetraveler, han2020dyernie, ding2022few}. On the other hand, the rule-based methods mine the temporal logical rules extracted and extract candidates directly on the temporal knowledge graphs\cite{liu2022tlogic}. 

\textbf{Investigating TKG with Language Models}
The semantic part stored in the temporal knowledge graphs is heavily overlooked in either embedding-based or rule-based temporal knowledge graph methods. Early explorers had tryouts in introducing language models in the TKG domain, some fused pre-trained language representations to the temporal knowledge embeddings~\citep{han2022enhanced}, and some flattened explicit temporal events with the emergent in-context learning ability of large language models however not comparable with conventional performance~\citep{lee2023temporal}. Other researchers had tryouts in combing KG with LLM, utilizing the knowledge-aware prompting method~\citep{baek-etal-2023-knowledge, rony2022dialokg,sun2023think,zhang2022drlk}, however, cannot be transferred to the tKG domain due to their ignorance of temporal characteristics.
